Single Underwater Image Restoration by Contrastive Learning

Underwater image restoration attracts significant attention due to its importance in unveiling the underwater world. This paper elaborates on a novel method that achieves state-of-the-art results for underwater image restoration based on the unsupervised image-to-image translation framework. We design our method by leveraging from contrastive learning and generative adversarial networks to maximize mutual information between raw and restored images. Additionally, we release a large-scale real underwater image dataset to support both paired and unpaired training modules. Extensive experiments with comparisons to recent approaches further demonstrate the superiority of our proposed method.

==> figures/pairdata.tex <==
\begin{figure}[htbp]
  \begin{minipage}[t]{0.46\linewidth} 
    \centering 
    \text{Raw image}
  \end{minipage} 
    \begin{minipage}[t]{0.46\linewidth} 
    \centering 
    \text{Restoration image}
    \end{minipage}
  \\
  \begin{minipage}[t]{0.46\linewidth} 
    \centering 
    \includegraphics[width=1.55in, height=1in]{figures/Capture1.PNG}
  \end{minipage} 
    \begin{minipage}[t]{0.46\linewidth} 
    \centering 
    \includegraphics[width=1.55in, height=1in]{figures/day3_site2_best1.png}
  \end{minipage} 
  \\
    \begin{minipage}[t]{0.46\linewidth} 
    \centering 
    \includegraphics[width=1.55in, height=1in]{figures/capture2.PNG}
  \end{minipage} 
    \begin{minipage}[t]{0.46\linewidth} 
    \centering 
    \includegraphics[width=1.55in, height=1in]{figures/day3_site2_best2.png}
  \end{minipage} 
  
  \caption{Results of restoration based on imaging model}
  \label{fig:pair}
\end{figure}
